On the connected (sub)partition polytope

Let $k$ be a positive integer and let $G$ be a graph with $n$ vertices. A connected $k$-subpartition of $G$ is a collection of $k$ pairwise disjoint sets (a.k.a. classes) of vertices in $G$ such that each set induces a connected subgraph. The connected $k$-subpartition polytope of $G$, denoted by $\poly(G,k)$, is defined as the convex hull of the incidence vectors of all connected $k$-subpartitions of $G$. Many applications arising in off-shore oil-drilling, forest planning, image processing, cluster analysis, political districting, police patrolling, and biology are modeled in terms of finding connected (sub)partitions of a graph. This study focuses on the facial structure of~$\poly(G,k)$ and the computational complexity of the corresponding separation problems. We first propose a set of valid inequalities having non-zero coefficients associated with a single class that extends and generalizes the ones in the literature of related problems, show sufficient conditions for these inequalities to be facet-defining, and design a polynomial-time separation algorithm for them. We also devise two sets of inequalities that consider multiple classes, prove when they define facets, and study the computational complexity of associated separation problems. Finally, we report on computational experiments showing the usefulness of the proposed inequalities.

==> runtime-bipartite-data.tex <==
719.17,180.52,16000.38,16000.06
356.15,242.32,16000.32,16000.06
16000.6,16000.1,16000.41,16000.14
16000.08,16000.02,16000.28,16000.08
16000.18,16000.19,16000.09,16000.1
16000.11,16000.33,16000.16,16000.05
747.53,16000.38,16000.29,16000.24
16000.86,16000.57,16000.19,16000.32
92.3,114.02,16000.39,16000.2
250.13,336,16000.2,16000.11
16000.57,16000.41,16000.13,16000.11
16000.34,16000.11,16000.42,16000.26
16000.04,16000.27,16000.48,16000.1
16000.03,16000.64,16000.45,16000.03
16000.86,16000.51,16000.06,16000.07
16000.53,16000.04,16000.16,16000.17
16000.57,16000.32,16000.19,16000.11
16000.91,16000.41,16000.02,16000.1
16000.13,16000.48,16000.34,16000.11
16000.21,16000.04,16000.24,16000.47
16000.02,16000.12,16000.02,93.78
16000.72,16000.16,16000.37,16000.12
16000.29,16000.44,16000.37,16000.01
16000.56,16000.65,16000.53,16000.16
16000.11,16000.13,810.92,16000.09
16000.36,16000.02,16000.35,16000.71
16000.13,16000.14,16000.07,16000.21
16000.24,16000.28,16000.14,16000.29
16000.31,16000.06,16000.76,16000.09
16000.86,16000.11,16000.37,16000.46
16000.03,16000.06,158.86,87.96
414.43,16000.15,16000.38,16000.08
16000.59,881.71,453.61,220.83
16000.03,16000.98,16000.19,16000.22
270.72,572.39,143.86,52.99
241.72,16000.5,16000.57,16000.3
459.4,16000.24,149.16,66.88
16000.23,16000.59,16000.06,16000.71
16000.02,16000.11,16000.22,16000.19
16000.56,16000.36,16000.73,16000.61
16000.48,16000.23,16000.21,848.92
16000.82,16000.78,16000.74,16000.24
16000.75,16000.18,563.26,16000.1
16000.57,16000.07,16000.06,16000.53
16000.65,16000.29,16000.36,16000.15
16000.28,16000.11,16000.23,16000.23
54.3,16000.17,134.08,85.13
64.51,342.71,16000.09,16000.31
16000.31,631.23,462.3,239.21
789.88,16000.1,112.42,16000.04
156.1,437.65,16000.09,16000.05
314.86,338.55,16000.15,958.59
184.54,595.43,270.86,16000.13
16000.48,16000.24,16000.61,16000.1
16000.49,16000.32,16000.06,16000.12
692.47,706.49,16000.39,16000.6
16000.35,16000.27,16000.32,16000.03
16000.05,16000.01,16000.23,16000.34
111.62,369.65,16000.02,16000.43
16000.17,16000.25,16000.07,16000.46
256.76,524.09,16000.01,16000.05
79.58,268.37,16000.45,16000.1
115.39,16000.08,16000.21,16000.7
434.15,170.07,16000.46,16000.64
44.48,247.59,16000.31,16000.07
16000.13,16000.69,16000.41,16000.29
16000.04,16000.02,16000.18,16000.98
769.45,16000.39,16000.01,16000.12
16000.34,16000.53,16000.44,16000.46
589.43,16000.48,16000.15,16000.2
98.14,313.81,415.41,16000.03
16000.31,16000.09,16000.23,16000.13
278.92,107.35,16000.1,16000.27
77.11,114.47,137,16000.26
16000.02,16000.03,16000.15,16000.25
16000.56,16000.43,16000.29,16000.82
534.67,16000.07,16000.22,16000.11
16000.82,16000.41,16000.19,16000.27
16000.46,559.38,16000.49,16000.17
83.14,295.56,205.39,16000.6
180.21,720.35,16000.55,16000.19
39.58,226.94,16000.67,16000.29
63.3,235.1,16000.1,16000.68
16000.06,16000.04,16000.21,16000.52
239.19,705.86,428.65,16000.18
67.44,314.55,115.8,16000.19
16000.75,16000,503.24,16000.16
137.11,16000.33,16000.9,16000.28
34.84,24.33,213.46,16000.23
16000.46,16000.42,16000.09,16000.14
225.74,16000.02,16000.07,16000.64
181.47,99.99,130.47,100.85
16000.51,16000.12,16000.49,16000.11
16000.24,405.83,158.21,16000.48
159.37,227.24,73.69,16000.38
59.16,137.67,111.16,16000.68
225.58,16000.1,52.94,16000.12
71.27,125.51,27.09,16000.13
16000.12,16000.29,355.92,16000.23
118.22,296.12,139.04,16000.87
64.45,73.63,17.21,16000.1
543.46,278.15,249.06,16000.05
22.07,876.13,16000.68,16000.02
37.83,57,101.05,41.31
48.97,16000.04,741.76,16000.62
163.55,50.12,16000.38,16000.13
12.59,74.15,106.17,16000.21
16000.39,16000.38,16000.33,16000.29
602.39,16000.93,140.74,16000.5
145.5,31.76,36.56,16000.15
897.15,16000.03,16000.98,16000.53
105.81,16000.07,133.99,16000.18
83.69,626.17,91.05,16000.01
16000.62,16000.71,16000,16000.34
16000.55,232.31,841.77,16000.6
77.93,68.16,16000.37,16000.12
219.97,372.95,97.48,16000.1
63.95,40.69,14.24,16000.55
191.88,2.21,15.44,16000.1
103.43,16000.95,353.48,16000.17
85.64,52.83,267.33,16000.79
31.83,12.58,81.03,16000.1
129.11,100.23,33.54,16000.14
36.34,646.17,30.02,16000.14
124.6,22.87,14.91,16000.05


==> runtime-bipartite-dense-data.tex <==
65.04,154.13,42.49,200.08
186.05,94.88,111.54,901.19
901.79,18.84,13.57,901.95
22.36,7.89,27.01,901.29
39.34,51.92,17.25,901.59
32.33,80.66,56.17,370.82
73.07,901.29,721.52,901.44
30.81,20.05,28.37,901
14.54,13.86,22.23,902.98
23.23,28.75,24.84,901.21
52.08,507.23,63.07,32
40.2,41.35,902,901.05
21.05,24.82,12.18,901.13
25.16,18,18.6,901.22
73.48,21.45,11.3,901.1
12.47,272.96,74.41,165.92
105.18,257.03,901.59,901.31
125.03,13.87,114.86,901.22
4.19,10.29,1.75,28.96
0.66,0.62,41.78,16.39
493.82,902.1,449.76,609.36
513.64,269.62,51.96,901.41
211.47,27.01,15.36,901.28
21.37,35.14,16.36,901.13
11.25,18.35,12.11,901.06
9.14,115.88,25.35,62.84
38.88,150.98,20.8,901.12
5.12,20.81,188.03,901.27
75.57,20.97,19.28,901.01
5.01,3.63,9.52,901.15
342.04,901.62,516.88,215.93
112.2,307.82,206.67,901.27
86.87,903.31,109.38,901.51
93.19,42.09,52.16,901.05
57.42,94.81,104.94,905.84
81.78,901.08,317.98,901.19
124.15,37.76,16.04,901.07
471.88,902.18,56.34,901.31
7.02,7.56,23.91,901.03
3.89,43.71,10.28,902.32
106,611.78,163.86,52.55
61.24,741.51,30.57,901.34
149.48,629.15,16.42,901.48
85.25,63.11,39.8,901.06
25.58,7.25,13.01,901.09
393.75,361,324.62,901.18
901.4,188.9,244.4,901.11
117.93,902.56,75.2,901.41
9.69,125.34,28.91,901.35
6.67,292.97,14.3,901.52
33.44,15.22,16.05,23.21
8.05,29.76,7.35,901.63
184.34,11.38,22.32,901.62
31.09,0.35,204.13,901.01
32.11,24.42,43,901.3
20.94,43.94,22.71,62.37
11.35,5.22,8.55,901
9.27,23.66,21.04,901.08
33.05,9.32,14.42,901.12
40.06,28.45,12.1,901.48
1.06,1.48,0.74,1.67
7.17,6.38,0.19,7.95
449.21,446.1,0.59,7.61
6.5,5.97,2.07,6.69
5.14,0.24,1.63,51.19
1.24,36.63,49.25,25.31
32.17,259.19,158.19,901.43
45.47,15.54,506.36,901.33
8.1,21.17,901.28,901.14
0.51,0.43,59.81,231.65
3.65,33.51,23.67,18.11
6.33,902.15,544.47,901.02
4.11,3.63,0.29,41.93
1.09,0.97,5.28,48.52
10.82,9.66,1.03,63.26
16.26,57.92,12.97,108.3
11.78,4.47,7.23,901.11
10.08,7.21,8.22,901.01
35.93,13.83,20.19,901.43
4.85,0.24,17.62,901.74
41.43,17,70.5,109.79
14.61,18.42,15.6,901.28
33.57,1.51,8.78,902.01
42.96,14.09,20.76,902.91
18.42,32.2,8.37,901.03
14.88,412.1,39.49,142.08
25.37,18.62,14.44,901.38
13.92,2.26,15.45,901.25
38.19,25.44,14.26,901.04
21.56,0.72,0.61,901.08
17.32,14.07,10.93,30.63
431.21,22.04,34.63,901.09
54.27,26.48,594.98,901.69
6.17,6.4,84.24,901.08
17.41,5.41,30.6,902.02
5.29,84.18,18.4,23.51
9.17,27.24,49.56,901.24
6.38,12.48,216.05,901.07
16.59,11.85,48.53,146.19
4.65,0.3,2.46,240.86
11.83,4.87,8.26,24.43
12.05,9.9,659.02,901.12
1.55,0.49,0.57,901.19
0.5,0.47,80.61,894.44
2.49,2.2,0.37,101.9
16.59,30.62,71.61,77.49
43.27,35.97,635.72,901.08
1.59,18.27,14.13,901.25
102.84,22.19,147.46,901.39
1.36,2.99,10.38,901.03
0.08,20.66,26.34,19.78
1.85,0.67,446.24,901.02
3.02,4.08,20.01,901.05
0.42,16.2,33.89,112.77
15.11,13.98,79.25,112.09
12.47,2.37,15.61,63.94
0.49,0.99,3.95,901.06
3.88,6.47,0.41,901.18
26.89,18.1,12.99,901.35
29.92,0.71,10.72,846.55
12.13,20.29,10.62,25.73
2.82,7.97,902.19,901.1
2.93,1.22,66.34,901.04
14,0.61,905.09,901.36
0.29,0.15,113.74,901.02


==> runtime-random-sparse-data-ext.tex <==
5.16,0.85,12.88,11.15
22.92,58.48,55.37,114.34
901.58,901.02,901.02,901.06
12.81,41.09,40.52,30.53
1.1,0.81,0.79,4.29
0.7,2.4,11.98,10.46
12.48,27.24,92.25,85
141.25,86.9,124.98,330.3
4.22,3.23,4.69,6.23
0.09,0.09,0.29,1.06
2.02,16.69,5.06,16.01
64.49,77.52,77.3,92.75
127.36,480.55,902.04,901.2
11.89,10.87,18.73,16.67
1.27,0.89,1.52,2.15
0.59,3.05,20.95,22.48
13.43,32.63,95.72,178.54
79.43,901.41,901.03,901.13
154.69,901.9,902.72,901.09
51.25,69.73,108.52,103.43
0.6,0.49,2.67,9.11
15.99,13.31,35.54,60.47
13.37,13.99,7.67,9.07
0.4,0.31,0.62,4.84
0.05,0.06,0.14,0.23
17.86,457.87,901.08,901.02
166.85,425.45,901.23,901.28
901.95,901.05,901.06,901.64
21.32,902.22,177.92,109.96
10.13,8.81,12.85,26.21
84.02,79.56,78.7,45.4
279.45,356.95,247.81,355.63
260.32,256.04,220.55,594.41
93.34,89.84,367.19,149.71
4.01,3.6,3.79,107.27
60.5,160.58,901.09,901.16
901.09,901.83,901.66,901.01
901.6,902.97,901.26,901.22
902.59,903.18,901.12,901.26
901.33,902.87,901.51,901.22
68.01,67.19,851.87,901.06
527.37,516.84,901.67,901.3
901.8,901.41,901.59,901.04
112.35,110.29,255.14,107.13
8.38,7.95,7.51,30.61
95.5,404.13,901.23,868.12
901.79,901.68,901.36,901.2
902.5,901.39,903.04,901.6
422.86,418.43,144.34,310.88
59.13,55.79,44.56,35.43
339.91,339.31,88.4,392.19
901.38,901.47,491.34,578.42
106.55,105.28,223.28,577.27
150.46,148.23,59.62,11.11
8.08,7.39,15.07,11.82
901.22,901.02,901.27,901.04
901.01,901.32,901.45,901.06
902.47,901.21,901.61,579.57
901.13,901.89,902.55,901.96
394.21,388.21,156.51,421.62
20.08,19.65,4.27,2.64
0.06,0.07,0.04,3.79
0.15,0.14,0.12,0.09
198.55,205.68,0.15,0.29
4.81,4.29,5.15,3.72
578.77,575.38,62.26,297.76
489.72,486.91,162.33,4.26
2.83,2.63,6.58,0.22
0.17,0.17,0.21,9.63
0.22,0.17,3.62,15.62
901.01,901.01,510.55,833.84
901.46,901.06,901.38,901.21
901.17,901.18,590.16,623.34
99.63,97.03,154.47,34.5
8.92,8.27,6.31,6.83
3.38,3.13,3.07,2.72
0.03,0.03,2.2,4.57
0.08,0.08,0.1,8.34
0.45,0.36,0.34,0.07
8.47,7.98,4.14,11.51
26.76,25.86,17.26,11.07
4.07,3.8,5.21,2.82
0.15,0.14,3.2,2.77
0.77,0.61,0.76,32.46
0.56,0.47,1.28,5.71
901.15,325.95,316.59,158.07
340.03,901.07,901.13,360.38
176.93,174.75,116.61,85.16
901.2,902.15,86.85,27.49
12.83,12.31,18.92,7.1
0.04,0.04,3.95,0.04
6.89,6.63,6.69,4.72
16.49,15.91,6.71,9.51
15.4,15.33,11.98,12.47
2.01,1.73,3.42,0.77
0.01,0.01,0.01,0.01
0.09,0.09,0.05,0.06
0.03,0.03,0.03,0.03
0.03,0.03,0.03,0.03
0.05,0.05,0.05,0.05
339.06,333.62,69.92,124.01
901.03,901.05,729.23,901.18
774.84,767.21,126.74,73.72
125.25,122.84,2.93,27.71
4.08,3.74,2.44,20.59
173.6,171.3,444.19,142.29
212.1,210.75,3.49,174.71
0.16,0.13,4.27,4.09
0.16,0.14,1.66,17.21
0.23,0.19,22.87,0.16
94.08,47.87,15.29,86.14
0.09,0.07,6.64,5.34
0.32,0.26,0.22,5.24
0.16,0.13,0.11,0.09
0.53,0.44,1.03,0.09
25.96,24.45,19.9,2.91
259.13,255.54,300.9,674.61
0.15,0.14,5.57,12.04
4.16,3.89,60.33,9.3
0.14,0.12,3.98,1.89
901.32,901.3,901.14,867.12
901.14,902.45,901.09,901.11
311.32,305.22,70.97,4.54
5.82,5.49,10.87,27.1
2.74,2.46,0.25,5.87
3.67,3.46,0.18,1.7
0.09,0.08,0.07,0.07
0.09,0.08,0.08,0.12
0.56,0.48,1.64,0.71
0.23,0.21,0.22,0.2
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.02,0.02,0.02,0.02
0.85,0.7,0.41,10.24
2.32,2.04,0.96,0.04
0.05,0.05,0.05,0.05
0.05,0.05,0.05,0.05
0.06,0.06,0.06,0.07
26.08,337.26,279.62,210.42
7.71,7.3,5.97,420.56
0.17,0.13,5.61,7.03
7.22,6.34,0.21,5.42
9.64,8.85,8.1,3.88
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.02
0.01,0.01,0.01,0.01
0.02,0.02,0.02,0.02
0.01,0.01,0.01,0.01
0.02,0.03,0.02,0.02
0.02,0.02,0.02,0.02
2.24,1.85,4.99,10.16
5.43,5.37,7.48,0.16
0.1,0.11,0.16,10.1
1.81,1.62,12.4,1.92
0.27,0.29,1.78,3.62
2.22,2.5,9.39,12.54
17.31,17.01,18.1,2.67
21.88,20.28,3.17,16.3
13.56,12.62,7.74,12.02
2.99,2.51,5.06,5.64
0.01,0.01,0.01,0.01
0.08,0.08,0.05,0.18
0.02,0.02,0.02,0.02
0.03,0.02,0.02,0.03
0.05,0.05,0.06,0.07
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.02,0.02,0.02,0.02
0.01,0.01,0.01,0.01
0.02,0.02,0.02,0.01
0.02,0.02,0.02,0.02
0.05,0.05,0.05,0.59
0.04,0.04,0.06,0.04
0.02,0.01,0.01,0.01
0.04,0.04,0.04,0.05
0.05,0.04,0.05,0.08
0.01,0.01,0.01,0.01
0.02,0.02,0.02,0.02
0.02,0.02,0.02,0.02
0.03,0.03,0.03,0.03
0.05,0.05,0.06,0.05
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.02,0.02,0.02,0.02
0.01,0.01,0.01,0.01
0.03,0.02,0.02,0.01
0.02,0.02,0.02,0.02
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.02,0.02,0.02,0.02
0.04,0.05,0.05,0.14
0.04,0.04,0.04,0.04
0.14,0.15,0.08,0.09
0.12,0.12,0.12,0.08
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.02,0.02,0.02,0.02
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01
0.01,0.01,0.01,0.01

